A theory of pictures for quasi-posets

The theory of pictures between posets is known to encode much of the combinatorics of symmetric group representations and related topics such as Young diagrams and tableaux. Many reasons, com-binatorial (e.g. since semi-standard tableaux can be viewed as double quasi-posets) and topological (quasi-posets identify with finite topolo-gies) lead to extend the theory to quasi-posets. This is the object of the present article.

==> arbresbinaires.tex <==
%Arbres binaires

\newcommand{\bun}{
\begin{picture}(5,5)(-2,0)
\put(0,0){\line(0,0){5}}
\end{picture}}

\newcommand{\bdeux}{
\begin{picture}(10,15)(-5,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\end{picture}}

\newcommand{\btroisun}{
\begin{picture}(25,22)(-14,5)
\drawline(0,0)(0,7)(-14,21)
\drawline(0,7)(7,14)
\drawline(-7,14)(0,21)
\end{picture}}
\newcommand{\btroisdeux}{
\begin{picture}(25,22)(-10,5)
\drawline(0,0)(0,7)(14,21)
\drawline(0,7)(-7,14)
\drawline(7,14)(0,21)
\end{picture}}

\newcommand{\bquatreun}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-6.3,10.7){$\vee$}
\put(-9.1,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatredeux}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-6.3,10.7){$\vee$}
\put(-3.5,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatretrois}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-0.7,10.7){$\vee$}
\put(-3.5,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatrequatre}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-0.7,10.7){$\vee$}
\put(2.1,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatrecinq}{
\begin{picture}(15,20)(-7,0)
\put(0,0){\line(0,1){5}}
\put(0,5){\line(2,1){10}}
\put(0,5){\line(-2,1){10}}
\put(-3,6.5){\line(0,1){5}}
\put(3,6.5){\line(0,1){5}}
\end{picture}}

%Arbres binaires décorés

\newcommand{\bddeux}[1]{
\begin{picture}(25,22)(-12,0)
\put(0,0){\line(0,0){10}}
\put(0,10){\line(1,1){10}}
\put(0,10){\line(-1,1){10}}
\put(-9,7){\tiny #1}
\end{picture}}

\newcommand{\bdtroisun}[2]{
\begin{picture}(25,22)(-14,5)
\drawline(0,0)(0,7)(-14,21)
\drawline(0,7)(7,14)
\drawline(-7,14)(0,21)
\put(-7,4){\tiny #1}
\put(-14,11){\tiny #2}
\end{picture}}

\newcommand{\bdtroisdeux}[2]{
\begin{picture}(25,22)(-10,5)
\drawline(0,0)(0,7)(14,21)
\drawline(0,7)(-7,14)
\drawline(7,14)(0,21)
\put(2,4){\tiny #1}
\put(9,11){\tiny #2}
\end{picture}}

\newcommand{\bddtroisun}[5]{
\begin{picture}(30,40)(-20,0)
\put(0,0){\line(0,0){10}}
\put(0,10){\line(1,1){10}}
\put(0,10){\line(-1,1){20}}
\put(-10,20){\line(1,1){10}}
\put(-9,7){\tiny #1}
\put(-19,17){\tiny #2}
\put(-21,32){\tiny #3}
\put(-1,32){\tiny #4}
\put(9,22){\tiny #5}
\end{picture}}
\newcommand{\bddtroisdeux}[5]{
\begin{picture}(30,40)(-10,0)
\put(0,0){\line(0,0){10}}
\put(0,10){\line(1,1){20}}
\put(0,10){\line(-1,1){10}}
\put(10,20){\line(-1,1){10}}
\put(3,7){\tiny #1}
\put(13,17){\tiny #2}
\put(-11,22){\tiny #3}
\put(-1,32){\tiny #4}
\put(19,32){\tiny #5}
\end{picture}}

